DuplexAct: How Interactive Are Frontier Full-Duplex Spoken Language Models?

End-to-end (E2E) full-duplex spoken language models (FD-SLMs) enable simutanous listening and speaking continously, requiring models to take appropriate interaction actions as conversations unfold. However, existing benchmarks lack a structured action-level formulation, often evaluate action occurrence rather than success, and provide limited coverage of diverse real-world conversations. We introduce DuplexAct, a benchmark for evaluating interaction action taking in E2E FD-SLMs. DuplexAct defines a three-level action taxonomy spanning eight interaction actions and 24 corresponding interaction conditions. We further characterize successful action-taking through immediate execution and subsequent follow-through, and develop action-specific evaluation metrics for both. DuplexAct contains 4,691 test instances spanning casual conversation, meetings, customer service, and interviews, including 2,531 instances derived from real-world conversational recordings. Together, DuplexAct provides a structured and real-world-grounded framework for systematically assessing how E2E FD-SLMs participate in ongoing spoken interaction.

==> Draft-components/Benchmark-results/03-Condition-Level-Analysis.tex <==
% ============================================================
\subsection{Condition-Level Analysis}
\label{sec:results_condition}
% ============================================================



==> Draft-components/history/01-Introduction-initial-update.tex <==
\begin{itemize}
    \item \textbf{Motivation: full-duplex interaction requires ongoing
    action taking.}
    During spoken interaction, a model must continually decide whether
    to speak, keep listening, continue its contribution, or respond to
    an intervention.
    These decisions determine how the model participates in the
    unfolding conversation.
    Understanding full-duplex interaction therefore requires evaluating
    the model's ability to take appropriate actions in context.

    \item \textbf{Evaluation goal: organise capabilities around actions.}
    An action-centred evaluation makes it possible to examine which
    interactional decisions a model handles successfully and under
    which conditions.
    This requires a structured action taxonomy, definitions of
    successful action taking, and tasks that elicit each action in
    relevant conversational situations.

    \item \textbf{Human interaction research provides the conceptual
    foundation.}
    Conversation Analysis (CA) and Interactional Linguistics examine
    how participants accomplish actions through situated contributions
    to conversation.
    Deppermann and Gubina describe action categorisation as sensitive
    to the analytical perspective, the practices used, and the
    sequential context \cite{deppermann_gubina_2026}.
    This motivates organising our taxonomy around the interactional
    coordination problems that participants need to manage.

    \item \textbf{Interactional competence identifies relevant
    capability domains.}
    Interactional competence (IC) brings these human interaction
    practices into the assessment of speaking
    \cite{roever_kasper_2018}.
    Galaczi and Taylor synthesise IC into five interconnected domains:
    turn management, topic management, interactive listening,
    breakdown repair, and non-verbal behaviour
    \cite{galaczi_taylor_2018}.

  \item \textbf{Deriving candidate actions from IC ability areas.}
We use the IC ability areas synthesised by Galaczi and Taylor
\cite{galaczi_taylor_2018} to identify coordination problems relevant
to our benchmark.
For each selected area, we examine the human interaction practices
described in CA and IC research and formulate candidate actions
that make these capabilities observable and testable:

\begin{itemize}
    \item \textbf{Turn management.}
    This area concerns how participants start, maintain, and end
    turns, including the management of pauses and interruptions.
    The coordination problem in our scope is deciding when to enter,
    defer, continue, or withdraw from speaking.
    These practices motivate the candidate actions
    \emph{wait, take turn, stop, hold floor, and interrupt}.

    \item \textbf{Interactive listening.}
    This area concerns how participants display recipiency and
    respond to another participant's ongoing contribution.
    The coordination problem in our scope is deciding whether
    incoming speech calls for a response and how to provide
    listener feedback while another participant continues.
    Listener-response practices motivate \emph{backchannel}.
    Research on participation roles and recipient selection
    further informs \emph{ignore}, addressing selective
    non-response to input that is irrelevant to the ongoing
    interaction \cite{clark_carlson_1982,lerner_2003}.

    \item \textbf{Breakdown repair and topic management.}
    These areas concern how participants address interactional
    trouble and organise the continuation or redirection of
    an activity.
    The coordination problem in our scope is continuing
    appropriately after an interruption or a contribution
    that changes the ongoing activity.
    Relevant practices motivate \emph{recover}, covering
    re-entry and adaptation of the model's next contribution.
\end{itemize}

This ability-to-problem-to-action derivation yields eight
candidate actions.
Together, they form a structured, representative taxonomy
for evaluating the selected aspects of interactional competence.

    \item \textbf{CA motivates a sequential definition of action
    success.}
    Actions are both \emph{context-sensitive} and
    \emph{context-renewing}: they respond to prior interaction and
    shape what becomes relevant next
    \cite{deppermann_gubina_2026}.
    Successful action taking therefore concerns how a contribution
    fits its current context and how the interaction proceeds
    following that contribution.

    \item \textbf{IC provides an assessment rationale for subsequent
    evidence.}
    IC research examines behaviour across the unfolding interaction
    to assess participants' abilities.
    For example, May et al.\ identify both immediate listener displays
    and subsequent responses that develop a partner's contribution
    as evidence relevant to interactive listening
    \cite{may_et_al_2020}.
    Later conduct can thus substantiate how an earlier contribution
    was understood and carried forward.

    \item \textbf{Action definitions specify two complementary
    aspects of successful performance.}
    Building on these perspectives, we define each action through:
    \begin{enumerate}
        \item \textbf{Immediate execution:}
        the behaviour and timing appropriate to the current
        interactional context.
        \item \textbf{Subsequent follow-through:}
        the later model behaviour that evidences appropriate
        continuation of the action.
    \end{enumerate}
    Relevant CA and IC accounts inform what each action accomplishes
    and which observable behaviours support its successful
    realisation.

    \item \textbf{Evaluation metrics follow the function of each
    action.}
    Immediate metrics measure whether the model performs the action
    at an appropriate moment.
    Subsequent metrics examine the specific behaviour expected
    following that action.
    For example, \emph{stop} combines speech cessation with maintained
    yielding, while \emph{hold floor} combines turn retention with
    appropriate adjustment of the ongoing contribution.
    Each metric therefore targets a defined aspect of the action's
    interactional function.

    \item \textbf{Task conditions instantiate the taxonomy.}
    We consolidate conversational conditions from existing benchmarks
    and develop additional cases to extend coverage of the selected
    coordination problems.
    Each task instantiates a general action in a concrete situation,
    with explicit contextual cues, expected behaviour, and an
    observation window.
    The resulting benchmark connects human interaction research,
    representative actions, task conditions, and action-specific
    evaluation criteria.
\end{itemize}

==> Draft-components/history/03-05-Evaluation.tex <==
\subsection{Evaluation}
% ============================================================
% Required packages
% ============================================================

% ============================================================
% Evaluation Overview Table
% ============================================================

% Required packages:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{tabularx}
% \usepackage{array}

\begin{table*}[t]
\centering
\caption{
Overview of the reliability-aware evaluation framework.
The base metric captures the directly observed interaction outcome,
while the reliability axis evaluates whether that outcome provides
sufficient evidence of successful action handling.
Timing metrics are reported as auxiliary diagnostics where applicable.
}
\label{tab:evaluation_overview}

\renewcommand{\arraystretch}{1.18}

\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{1.35cm}
    >{\raggedright\arraybackslash}p{2.15cm}
    >{\raggedright\arraybackslash}p{2.35cm}
    >{\raggedright\arraybackslash}p{2.55cm}
    X
}
\toprule

\textbf{Level 1 Action}
&
\textbf{Level 2 Action}
&
\textbf{Base Metric}
&
\textbf{Timing Metric}
&
\textbf{Reliability Axis}
\\

\midrule

% ============================================================
% Silent Actions
% ============================================================

\multirow{3}{*}{Silent}
&
Wait
&
Silence Rate (SR)
&
--
&
Post-Wait Response Rate (auto)
\\

\cmidrule(lr){2-5}

&
Stop
&
Yield Rate (YR)
&
Yield Latency
&
Floor-Release Validity Score (LLM)
\\

\cmidrule(lr){2-5}

&
Ignore
&
Silence Rate (SR)
&
--
&
Post-Event Response Rate (auto); Context-Ignore Score (LLM)
\\

\midrule

% ============================================================
% Speak Actions
% ============================================================

\multirow{5}{*}{Speak}
&
Smooth Turn Taking
&
Take-Over Rate (TOR)
&
Response Latency
&
Relevance Score (LLM); Completeness Score (LLM); Helpfulness Score (LLM)
\\

\cmidrule(lr){2-5}

&
Hold Floor
&
Floor-Holding Rate (FHR)
&
--
&
Intent Continuation Score (LLM); Semantic Steering Score (LLM)
\\

\cmidrule(lr){2-5}

&
Interrupt User
&
Take-Over Rate (TOR)
&
Interruption Latency
&
Content Validity Score (LLM); Position Validity Score (LLM)
\\

\cmidrule(lr){2-5}

&
Backchannel
&
Backchannel Rate (BCR)
&
Backchannel Timing
&
Context/Scenario Alignment; Next-Turn Verification
\\

\cmidrule(lr){2-5}

&
Respond \& Recover
&
Take-Over Rate (TOR)
&
Response Latency
&

Recover type match score (LLM); 
Address interruption Score (LLM); 
Natural reentry Score (LLM);
Return-to-thread Score (LLM)
\\

\bottomrule
\end{tabularx}

\end{table*}
\paragraph{Base metrics.}
For each action $a$, let $N_a$ denote the number of evaluation samples
constructed for that action. The base metrics quantify whether the expected
observable interaction behavior occurs in these samples:

\begin{itemize}
    \item \textbf{Take-Over Rate (TOR):}
    proportion of samples in which the system takes the floor within the
    predefined action-specific interval,
    \[
    \mathrm{TOR}
    =
    \frac{\#\{\text{samples with takeover in the predefined interval}\}}
         {N_a}.
    \]
    TOR is used for \textit{Smooth Turn Taking}, \textit{Interrupt User},
    and \textit{Respond \& Recover}. The predefined interval is specified
    by the corresponding action condition.
    
    \item \textbf{Silence Rate (SR):}
    proportion of samples in which the system does not take over the floor
    within the predefined interval,
    \[
    \mathrm{SR}
    =
    \frac{\#\{\text{samples with no takeover in the predefined interval}\}}
         {N_a}
    =
    1-\mathrm{TOR}.
    \]
    We use SR for \textit{Wait} and \textit{Ignore}, where remaining silent
    is the expected observable behavior.

    \item \textbf{Yield Rate (YR):}
    proportion of samples in which the system successfully relinquishes the
    floor within the predefined yield interval,
    \[
    \mathrm{YR}
    =
    \frac{\#\{\text{samples with a successful floor yield in the predefined interval}\}}
         {N_{\mathrm{Stop}}}.
    \]

    \item \textbf{Floor-Holding Rate (FHR):}
    proportion of samples in which the system successfully retains the
    conversational floor when it is expected to continue speaking,
    \[
    \mathrm{FHR}
    =
    \frac{\#\{\text{samples with successful floor retention}\}}
         {N_{\mathrm{HoldFloor}}}.
    \]

    \item \textbf{Backchannel Rate (BCR):}
    proportion of backchannel samples in which the system produces at least one backchannel,
    \[
    \mathrm{BCR}
    =
    \frac{\#\{\text{samples with at least one backchannel}\}}
         {N_{\mathrm{Backchannel}}}.
    \]

\end{itemize}


\paragraph{Timing metrics.}
Timing metrics complement the base success rates by characterizing when the corresponding interaction behavior occurs. For each sample $i$, we define the relevant event timestamps according to the evaluated action.

\begin{itemize}

    \item \textbf{Yield Latency.}
    For \textit{Stop}, let $t_i^{\mathrm{user,start}}$ denote the onset of the user interruption and $t_i^{\mathrm{model, end}}$ denote the time at which the system stops its current response and yields the floor. Yield latency is

    \[
    L_i^{\mathrm{yield}}
    =
    t_i^{\mathrm{model, end}}
    -
    t_i^{\mathrm{user,start}}.
    \]

    A smaller value indicates that the system yields the floor more quickly after the user begins interrupting.

    \item \textbf{Response Latency.}
    Let $t_i^{\mathrm{user,end}}$ denote the end of the user's turn and $t_i^{\mathrm{model,start}}$ denote the onset of the system response. Response latency is defined as

    \[
    L_i^{\mathrm{response}}
    =
    t_i^{\mathrm{model,start}}
    -
    t_i^{\mathrm{user,end}}.
    \]

    Positive values indicate that the system starts responding after the user finishes, whereas negative values indicate that the system starts responding before the end of the user's turn. The magnitude of the negative latency reflects how early the response begins relative to the user's turn completion.

    \item \textbf{Interruption Latency.}
    Let $t_i^{\mathrm{int}}$ denote the predefined appropriate interruption point and $t_i^{\mathrm{model,start}}$ denote the onset of the system interruption. Interruption timing is defined as

    \[
    \Delta_i^{\mathrm{int}}
    =
    t_i^{\mathrm{model,start}}
    -
    t_i^{\mathrm{int}}.
    \]

    A negative value indicates that the system interrupts before the predefined target point, whereas a positive value indicates that the system interrupts after the target point.

    \item \textbf{Backchannel Timing.}
    Let $t_i^{\mathrm{bc}}$ denote the predefined target point for backchanneling. If the model emits one or more valid backchannels in sample $i$, let $t_{i,1}^{\mathrm{model,start}}$ denote the onset of the first valid backchannel. Backchannel timing is defined as

    \[
    \Delta_i^{\mathrm{bc}}
    =
    t_{i,1}^{\mathrm{model,start}}
    -
    t_i^{\mathrm{bc}}.
    \]

    A negative value indicates that the first valid backchannel is emitted before the predefined target point, whereas a positive value indicates that it is emitted after the target point. If no valid backchannel is emitted, the backchannel timing is undefined for that sample and the failure is instead captured by the Backchannel Rate (BCR).

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\captionsetup{font=footnotesize}
\caption{
Candidate full-duplex spoken dialogue systems considered in our evaluation.
Conversation-control level follows the survey taxonomy:
\textbf{L0} denotes duplex control through an external controller or orchestration mechanism;
\textbf{L1} denotes a dedicated duplex predictor operating on internal LLM representations;
and \textbf{L2} denotes duplex decisions represented directly within the model's generation/token stream.
For proprietary systems whose internal control mechanism is not disclosed, ``--'' is reported.
}
\label{tab:benchmark_candidates}
\resizebox{\textwidth}{!}{
\begin{tabular}{l l l l c l}
\toprule
\textbf{Model} &
\textbf{Year / Venue} &
\textbf{Institute} &
\textbf{Model Size} &
\textbf{Control} &
\textbf{Existing Benchmark Evaluation} \\
\midrule

\multicolumn{6}{l}{\textbf{Open-source systems}} \\
\midrule

Moshi
& 2024 (Tech. Report)
& Kyutai
& 7B
& L2
& FDB v1, v1.5, v2; HumDial; FD-Bench; MTR \\

Freeze-Omni
& 2024 (ICML 2025)
& VITA / Tencent Youtu et al.
& 7B + speech modules
& L1
& FDB v1, v1.5, v2; HumDial; FD-Bench; MTR \\

Mini-Omni2
& 2024 (Tech. Report)
& gpt-omni
& 0.5B + speech/vision modules
& L2
& -- \\

VITA-1.5
& 2025 (NeurIPS 2025)
& VITA / Tencent et al.
& 7B + multimodal modules
& L0
& FD-Bench \\

Voila-autonomous
& 2025 (Tech. Report)
& Maitrix.org / UCSD / MBZUAI
& 8B
& L2
& -- \\

FLM-Audio
& 2026 (Tech. Report)
& CofeAI et al.
& 8B
& L2
& -- \\

Raon-SpeechChat
& 2026 (Tech. Report)
& KRAFTON
& 10B
& L2
& -- \\

NVIDIA Nemotron 3 VoiceChat
& 2026
& NVIDIA
& 11B
& L2
& -- \\

BayLing-Duplex
& 2026
& ICT, CAS
& 9B-class
& L2
& -- \\

Lychee-FD
& 2026 (ACL 2026)
& HIT-Shenzhen / Tencent / CUHK-Shenzhen et al.
& $\sim$7B-class
& L2
& -- \\

DuplexOmni
& 2026
& XJTU / PKU / Meituan
& 35B
& L1
& -- \\

MiniCPM-o 4.5
& 2026 (Tech. Report)
& OpenBMB / ModelBest / Tsinghua et al.
& 9B
& L2
& -- \\

\midrule
\multicolumn{6}{l}{\textbf{Closed-source systems}} \\

Gemini 3.1 Flash Live
& -- & Google & -- & --
& FDB v3; $\tau$-Voice \\

GPT-Realtime-2.1
& -- & OpenAI & -- & --
& -- \\

Amazon Nova 2 Sonic
& -- & Amazon & -- & --
& -- \\

Grok Voice
& -- & xAI & -- & --
& FDB v3; $\tau$-Voice \\

Qwen3.5-Omni-Flash-Realtime
& -- & Alibaba Cloud & -- & --
& -- \\

\bottomrule
\end{tabular}
}
\end{table*}

\end{itemize}

==> Draft-components/history/03-07-Realistic_data.tex <==
\subsubsection{Natural data}
\begin{table}[t]
\centering
\caption{Overview of realistic data coverage extracted from real-world corpora.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllc}
\toprule
\textbf{L2 Action} & 
\textbf{L3 Action} & 
\textbf{Scenario Coverage} &
\textbf{Samples} \\
\midrule

\multirow{3}{*}{Wait}
& Wait within intra-sentential pause
& Casual, Interview, Customer Service, Meeting
& 200 \\
& Wait at inter-sentential boundary
& Casual, Interview, Customer Service, Meeting
& 200 \\
& Wait for continued content
& Casual, Interview, Customer Service, Meeting
& 200 \\

\midrule

Stop
& Stop immediately mid-sentence
& Casual, Interview, Customer Service, Meeting
& 200 \\

\midrule

Take Turn
& Take turn with slight overlap
& Casual, Interview, Meeting
& 200 \\

\midrule

\multirow{3}{*}{Hold Floor}
& Continue current answer
& Casual, Interview, Customer Service, Meeting
& 200 \\
& Continue but shorten
& Casual, Interview, Customer Service, Meeting
& 131 \\
& Continue with simplification
& Casual, Interview, Customer Service, Meeting
& 200 \\

\midrule

\multirow{2}{*}{Backchannel}
& Signal acknowledgement / understanding / agreement
& Casual, Interview, Customer Service, Meeting
& 200 \\
& Signal uncertainty
& Casual, Interview, Customer Service, Meeting
& 200 \\

\midrule

\multirow{3}{*}{Respond \& Recover}
& Correct
& Casual, Interview, Customer Service, Meeting
& 200 \\
& Enrich
& Casual, Interview, Customer Service, Meeting
& 200 \\
& Shift topic
& Casual, Interview, Customer Service, Meeting
& 200 \\

\midrule

\multicolumn{3}{r}{\textbf{Total}}
& \textbf{2531}\\

\bottomrule
\end{tabular}
}
\label{tab:realistic_data_overview}
\end{table}


\begin{table*}[t]
\centering
\caption{
Overall interaction-action performance under the two evaluation protocols.
%Timing (\textbf{T}) is reported as median seconds.
}
\label{tab:main_results}

\scriptsize
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.15}

% ============================================================
% (a) Direct Replay
% ============================================================

\textbf{(a) Direct Replay}

\vspace{3pt}

\begin{tabular}{lcccc}
\toprule
\textbf{Model}
& \makecell{\textbf{Wait}\\
  \scriptsize I$\uparrow$ / S$\uparrow$}
& \makecell{\textbf{Ignore}\\
  \scriptsize I$\uparrow$ / S$\uparrow$}
& \makecell{\textbf{Take Turn}\\
  \scriptsize I$\uparrow$ / S$\uparrow$}
& \makecell{\textbf{Backchannel}\\
  \scriptsize I$\uparrow$ / S$\uparrow$}
\\
\midrule

\multicolumn{5}{l}{\textit{Open-source models}} \\
\midrule

Moshi
& 82.2 / 45.6
& 32.5 / 89.2
& 36.2 / 19.4
& 6.2 / 60.0
\\

Freeze-Omni
& 73.2 / 23.2
& 61.5 / 9.8
& 10.2 / 47.5
& 0.2 / 0.0
\\

Mini-Omni2
& 8.7 / 32.7
& 11.8 / 2.1
& 12.0 / 15.3
& 0.0 / n/a
\\

VITA-1.5
& 91.8 / 64.4& 55.5 / 91.4& 8.0 / 27.1& 0.0 / n/a\\

Voila-Autonomous
& 96.2 / 45.8
& 99.0 / 82.6
& 44.3 / 20.3
& 1.5 / 33.3
\\

FLM-Audio
& 95.5 / 18.3
& 84.2 / 87.5
& 35.2 / 3.8
& 0.2 / 0.0
\\

Raon-SpeechChat
& 51.7 / 70.3
& 47.0 / 79.8
& 65.2 / 23.0
& 31.0 / 43.5
\\

BayLing-Duplex
& 92.8 / 31.2
& 78.0 / 91.3
& 11.7 / 10.0
& 0.2 / 0.0
\\

Lychee-FD
& 98.2 / 53.1
& 80.8 / 97.5
& 20.8 / 10.4
& 2.2 / 22.2
\\

MiniCPM-o 4.5
& 95.2 / 74.4
& 72.8 / 83.8
& 37.8 / 43.2
& 2.5 / 70.0
\\

\midrule
\multicolumn{5}{l}{\textit{Close-source models}} \\
\midrule

Gemini 3.1 Flash Live
& 98.0 / 85.4
& 79.0 / 81.3
& 38.3 / 82.2
& 1.0 / 50.0
\\

GPT-Realtime-2.1
& 99.8 / 95.7
& 93.5 / 73.8
& 27.5 / 83.0
& 0.2 / 100.0
\\

Grok Voice
& 99.2 / 74.3
& 98.5 / 75.4
& 30.3 / 81.9
& 0.8 / 33.3
\\

Qwen3.5-Omni-Flash-Realtime
& 89.3 / 90.5
& 68.5 / 79.9
& 41.3 / 78.6
& 3.8 / 86.7
\\

\bottomrule
\end{tabular}

\vspace{9pt}

% ============================================================
% (b) Simulator Replay
% ============================================================

\textbf{(b) Simulator Replay}

\vspace{3pt}

\begin{tabular}{lcccc}
\toprule

\textbf{Model}
&
\makecell{
\textbf{Stop}\\
\scriptsize I$\uparrow$ / T$\downarrow$ / S$\uparrow$
}
&
\makecell{
\textbf{Hold Floor}\\
\scriptsize I$\uparrow$ / S$\uparrow$
}
&
\makecell{
\textbf{Interrupt}\\
\scriptsize I$\uparrow$ / T / S$\uparrow$
}
&
\makecell{
\textbf{Recover}\\
\scriptsize I$\uparrow$ / T / S$\uparrow$
}
\\

\midrule

\multicolumn{5}{l}{\textit{Open-source models}} \\
\midrule

Moshi
& 98.0 / 0.96 / 70.7
& 46.8 / 58.1
& 67.5 / $-3.97$ / 0.0
& 61.1 / 1.32 / 28.0
\\

Freeze-Omni
& 94.7 / 1.80 / 100.0
& 82.4 / 50.0
& 25.5 / $-8.85$ / 19.6
& 5.8 / 2.15 / 48.6
\\

FLM-Audio
& 97.3 / 4.13 / 100.0
& 75.8 / 65.4
& 2.8 / $-5.84$ / 0.0
& 4.1 / 4.52 / 14.3
\\

Raon-SpeechChat
& 95.1 / 5.20 / 93.1
& 91.9 / 26.1
& 36.8 / $-8.30$ / 0.0
& 14.4 / 2.72 / 7.2
\\

BayLing-Duplex
& 98.8 / 3.05 / 93.2
& 82.9 / 26.5
& 29.2 / $-2.91$ / 0.0
& 49.0 / 3.56 / 16.6
\\

MiniCPM-o 4.5
& 98.2 / 3.47 / 98.8
& 85.8 / 49.6
& 9.8 / $-4.49$ / 17.9
& 44.4 / 2.43 / 66.9
\\

\midrule

\multicolumn{5}{l}{\textit{Close-source models}} \\
\midrule

Gemini 3.1 Flash Live
& 100.0 / 1.74 / 100.0
& 70.0 / 57.3
& 1.8 / $-5.48$ / 14.3
& 97.0 / 2.56 / 78.6
\\

GPT-Realtime-2.1
& 100.0 / 1.61 / 100.0
& 57.2 / 39.3
& 8.8 / $-7.27$ / 8.6
& 77.7 / 3.00 / 90.3
\\

Grok Voice
& 100.0 / 2.37 / 96.7
& 67.8 / 49.4
& 0.0 / n/a / n/a
& 80.5 / 3.13 / 84.0
\\

Qwen3.5-Omni-Flash-Realtime
& 100.0 / 2.41 / 98.3
& 72.5 / 49.6
& 2.2 / $-4.94$ / 66.7
& 91.3 / 2.68 / 84.9
\\

\bottomrule
\end{tabular}

\vspace{3pt}

\footnotesize
\textit{Notation:}
\texttt{n/a} indicates that no applicable observation is available.

\end{table*}

==> Draft-components/history/03-08-Synthesize_data.tex <==
\subsubsection{Synthesize data}
\begin{table}[t]
\centering
\caption{Overview of synthesized data coverage.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllcl}
\toprule
\textbf{L2 Action} & 
\textbf{L3 Action} & 
\textbf{Scenario Coverage} & 
\textbf{Topic / Setting Coverage} & 
\textbf{Samples} \\
\midrule

\multirow{2}{*}{Hold Floor}
& Continue with other-directed speech
& Casual, Meeting, Interview, Customer Service
& Setting-based (10 settings/scenario)
& 200 \\
& Continue with background speech
& Casual, Meeting, Interview, Customer Service
& Setting-based (10 settings/scenario)
& 200 \\

\midrule

\multirow{3}{*}{Respond and Recover}
& Shorten response after interruption
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
& Repeat response after interruption
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
& Ask follow-up after interruption
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\

\midrule

\multirow{2}{*}{Ignore}
& Ignore background speech during user speech
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
& Ignore other-directed speech during user speech
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\

\midrule

\multirow{2}{*}{Take Turn}
& Take turn immediately
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
& Take turn with delay
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\

\midrule

\multirow{2}{*}{Interrupt User}
& Interrupt for help
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
& Interrupt for safety
& N/A
& Hazard-based (10 hazard types)
& 200\\

\midrule
\multicolumn{4}{r}{\textbf{Total}}
& \textbf{2200}\\

\bottomrule
\end{tabular}
}
\end{table}

==> Draft-components/history/03-Our_benchmark_initial.tex <==
\section{Benchmark Design}
\subsection{Overview}
\subsection{Action Space Coverage}
\subsection{Conversation Scenario Coverage}
\subsection{Interaction Design}
\input{Draft-components/03-05-Evaluation}
\subsection{Data Curation}

\begin{table}[t]
\centering
\caption{Overview of synthetic and realistic data coverage.}
\renewcommand{\arraystretch}{1.25}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllc}
\toprule
\textbf{Source} &
\textbf{L2 Action} &
\textbf{L3 Action} &
\textbf{Scenario Coverage} &
\textbf{Context Coverage} &
\textbf{Samples} \\
\midrule

\multirow{11}{*}{Synthetic}

& \multirow{2}{*}{Hold Floor}
& Continue with other-directed speech
& Casual, Meeting, Interview, Customer Service
& Setting-based (10 settings/scenario)
& 200 \\
&
& Continue with background speech
& Casual, Meeting, Interview, Customer Service
& Setting-based (10 settings/scenario)
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{3}{*}{Respond \& Recover}
& Shorten response after interruption
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
&
& Repeat response after interruption
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
&
& Ask follow-up after interruption
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{2}{*}{Ignore}
& Ignore background speech during user speech
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
&
& Ignore other-directed speech during user speech
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{2}{*}{Take Turn}
& Take turn immediately
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
&
& Take turn with delay
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{2}{*}{Interrupt User}
& Interrupt for help
& Casual, Meeting, Interview, Customer Service
& Topic-based (5 topics/scenario)
& 200 \\
&
& Interrupt for safety
& N/A
& Hazard-based (10 hazard types)
& 200\\

\midrule

\multirow{3}{*}{Real-world}

& \multirow{3}{*}{Wait}
& Wait within intra-sentential pause
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\
&
& Wait at inter-sentential boundary
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\
&
& Wait for continued content
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\

\cline{2-6}
\addlinespace

& Stop
& Stop immediately mid-sentence
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\

\cline{2-6}
\addlinespace

& Take Turn
& Take turn with slight overlap
& Casual, Interview, Meeting
& Corpus extracted
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{3}{*}{Hold Floor}
& Continue current answer
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\
&
& Continue but shorten
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 131 \\
&
& Continue with simplification
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{2}{*}{Backchannel}
& Signal acknowledgement / understanding / agreement
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\
&
& Signal uncertainty
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\

\cline{2-6}
\addlinespace

& \multirow{3}{*}{Respond \& Recover}
& Correct
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\
&
& Enrich
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\
&
& Shift topic
& Casual, Interview, Customer Service, Meeting
& Corpus extracted
& 200 \\

\midrule

\multicolumn{5}{r}{\textbf{Total}}
& \textbf{4731}\\

\bottomrule
\end{tabular}
}
\label{tab:data_overview}
\end{table}

\input{Draft-components/03-07-Realistic data}
\input{Draft-components/03-08-Synthesize data}
\subsubsection{Validation}

==> Draft-components/history/05-Results.tex <==
\section{Results}
\subsection{Main results}
% ============================================================
% Main Results: Base + Reliability
% ============================================================

% Required packages:
% \usepackage{booktabs}
% \usepackage{makecell}
% \usepackage{graphicx}

\begin{table*}[t]
\centering
\caption{
Main benchmark results across the eight Level-2 interaction actions.
For each action, \textbf{B} denotes the action-specific base metric,
\textbf{T} denotes the corresponding timing metric where applicable,
and \textbf{R} denotes the aggregated reliability score.
Timing metrics are defined in Table~\ref{tab:evaluation_overview}.
}
\label{tab:main_results}

\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\textwidth}{!}{
\begin{tabular}{
    l
    c c c
    c c c c c
}
\toprule

\textbf{Model}
&
\makecell{
\textbf{Wait}\\
SR\\
\scriptsize B / R
}
&
\makecell{
\textbf{Stop}\\
YR\\
\scriptsize B / T / R
}
&
\makecell{
\textbf{Ignore}\\
SR\\
\scriptsize B / R
}
&
\makecell{
\textbf{Turn}\\
TOR\\
\scriptsize B / T / R
}
&
\makecell{
\textbf{Hold}\\
FHR\\
\scriptsize B / R
}
&
\makecell{
\textbf{Interrupt}\\
TOR\\
\scriptsize B / T / R
}
&
\makecell{
\textbf{BC}\\
BCR\\
\scriptsize B / T / R
}
&
\makecell{
\textbf{Recover}\\
TOR\\
\scriptsize B / T / R
}
\\

\midrule

\multicolumn{9}{l}{\textit{Open-source systems}} \\
\midrule

Moshi
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

Freeze-Omni
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

Mini-Omni2
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

VITA-1.5
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

Voila-autonomous
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

FLM-Audio
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

Rasa-SpeechChat
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

NVIDIA Nemotron 3 VoiceChat
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

HayLing-Duplex
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

Lychee-FD
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

DuplexOmni
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

MiniCPM-o 4.5
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

\midrule

\multicolumn{9}{l}{\textit{Closed-source systems}} \\
\midrule

Gemini 3.1 Flash Live
& 98.2 / 89.0& -- / -- / --
& 90.0 / 86.0& 27.2 / --/ --& -- / --
& -- / -- / --
& 3.3 / -- / --& -- / -- / --
\\

GPT-Realtime-2.1
& 99.8 / 70.0& -- / -- / --
& 98.0 / 78.1& 35.7 / -- / --& -- / --
& -- / -- / --
& 1.5 / -- / --& -- / -- / --
\\

Amazon Nova 2 Sonic
& -- / --& -- / -- / --
& -- / --
& -- / -- / --& -- / --
& -- / -- / --
& -- / -- / --
& -- / -- / --
\\

Grok Voice
& 99.7 / 20.0& -- / -- / --
& 99.5 / 59.4& 9.5 / -- / --& -- / --
& -- / -- / --
& 0.25 / -- / --& -- / -- / --
\\

Qwen3.5-Omni-Flash-Realtime
& 95.9 / 46.0& -- / -- / --
& 86.8 / 62.5& 18.2 / -- / --& -- / --
& -- / -- / --
& 1.75 / -- / --& -- / -- / --
\\

\bottomrule
\end{tabular}
}

\vspace{2pt}

\footnotesize
\textit{Notation:}
B = Base;
T = Timing;
R = Reliability;
SR = Silence Rate;
YR = Yield Rate;
TOR = Take-Over Rate;
FHR = Floor-Holding Rate;
BCR = Backchannel Rate.
For actions without an explicit timing metric, entries are reported as
\textbf{B / R}; otherwise, entries are reported as
\textbf{B / T / R}.

\end{table*}

\vspace{-5pt}
\label{tab:main_results}

\scriptsize
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.05}

\begin{tabular}{lcccc}
\toprule

% ============================================================
% (a) Direct Replay
% ============================================================

\multicolumn{5}{c}{\textbf{(a) Direct Replay}} \\
\midrule

\textbf{Model}
& \makecell{\textbf{Wait}\\[-1pt]\scriptsize I$\uparrow$ / S$\uparrow$}
& \makecell{\textbf{Ignore}\\[-1pt]\scriptsize I$\uparrow$ / S$\uparrow$}
& \makecell{\textbf{Take Turn}\\[-1pt]\scriptsize I$\uparrow$ / S$\uparrow$}
& \makecell{\textbf{Backchannel}\\[-1pt]\scriptsize I$\uparrow$ / S$\uparrow$}
\\
\midrule

\multicolumn{5}{l}{\textit{Open-source models}} \\

Moshi
& 82.2 / 45.6
& 32.5 / 89.2
& 36.2 / 19.4
& 6.2 / 60.0
\\

Freeze-Omni
& 73.2 / 23.2
& 61.5 / 9.8
& 10.2 / 47.5
& 0.2 / 0.0
\\

Mini-Omni2
& 8.7 / 32.7
& 11.8 / 2.1
& 12.0 / 15.3
& 0.0 / n/a
\\

VITA-1.5
& 91.8 / 64.4
& 55.5 / 91.4
& 8.0 / 27.1
& 0.0 / n/a
\\

Voila-Autonomous
& 96.2 / 45.8
& 99.0 / 82.6
& 44.3 / 20.3
& 1.5 / 33.3
\\

FLM-Audio
& 95.5 / 18.3
& 84.2 / 87.5
& 35.2 / 3.8
& 0.2 / 0.0
\\

Raon-SpeechChat
& 51.7 / 70.3
& 47.0 / 79.8
& 65.2 / 23.0
& 31.0 / 43.5
\\

BayLing-Duplex
& 92.8 / 31.2
& 78.0 / 91.3
& 11.7 / 10.0
& 0.2 / 0.0
\\

Lychee-FD
& 98.2 / 53.1
& 80.8 / 97.5
& 20.8 / 10.4
& 2.2 / 22.2
\\

MiniCPM-o 4.5
& 95.2 / 74.4
& 72.8 / 83.8
& 37.8 / 43.2
& 2.5 / 70.0
\\

\midrule
\multicolumn{5}{l}{\textit{Close-source models}} \\

Gemini 3.1 Flash Live
& 98.0 / 85.4
& 79.0 / 81.3
& 38.3 / 82.2
& 1.0 / 50.0
\\

GPT-Realtime-2.1
& 99.8 / 95.7
& 93.5 / 73.8
& 27.5 / 83.0
& 0.2 / 100.0
\\

Grok Voice
& 99.2 / 74.3
& 98.5 / 75.4
& 30.3 / 81.9
& 0.8 / 33.3
\\

Qwen3.5-Omni-Flash-Realtime
& 89.3 / 90.5
& 68.5 / 79.9
& 41.3 / 78.6
& 3.8 / 86.7
\\

% ============================================================
% (b) Simulator Replay
% ============================================================

\midrule
\multicolumn{5}{c}{\textbf{(b) Simulator Replay}} \\
\midrule

\textbf{Model}
&
\makecell{\textbf{Stop}\\[-1pt]\scriptsize I$\uparrow$ / T$\downarrow$ / S$\uparrow$}
&
\makecell{\textbf{Hold Floor}\\[-1pt]\scriptsize I$\uparrow$ / S$\uparrow$}
&
\makecell{\textbf{Interrupt}\\[-1pt]\scriptsize I$\uparrow$ / T / S$\uparrow$}
&
\makecell{\textbf{Recover}\\[-1pt]\scriptsize I$\uparrow$ / T / S$\uparrow$}
\\
\midrule

\multicolumn{5}{l}{\textit{Open-source models}} \\

Moshi
& 98.0 / 0.96 / 70.7
& 46.8 / 58.1
& 67.5 / $-3.97$ / 0.0
& 61.1 / 1.32 / 28.0
\\

Freeze-Omni
& 94.7 / 1.80 / 100.0
& 82.4 / 50.0
& 25.5 / $-8.85$ / 19.6
& 5.8 / 2.15 / 48.6
\\

FLM-Audio
& 97.3 / 4.13 / 100.0
& 75.8 / 65.4
& 2.8 / $-5.84$ / 0.0
& 4.1 / 4.52 / 14.3
\\

Raon-SpeechChat
& 95.1 / 5.20 / 93.1
& 91.9 / 26.1
& 36.8 / $-8.30$ / 0.0
& 14.4 / 2.72 / 7.2
\\

BayLing-Duplex
& 98.8 / 3.05 / 93.2
& 82.9 / 26.5
& 29.2 / $-2.91$ / 0.0
& 49.0 / 3.56 / 16.6
\\

MiniCPM-o 4.5
& 98.2 / 3.47 / 98.8
& 85.8 / 49.6
& 9.8 / $-4.49$ / 17.9
& 44.4 / 2.43 / 66.9
\\

\midrule
\multicolumn{5}{l}{\textit{Close-source models}} \\

Gemini 3.1 Flash Live
& 100.0 / 1.74 / 100.0
& 70.0 / 57.3
& 1.8 / $-5.48$ / 14.3
& 97.0 / 2.56 / 78.6
\\

GPT-Realtime-2.1
& 100.0 / 1.61 / 100.0
& 57.2 / 39.3
& 8.8 / $-7.27$ / 8.6
& 77.7 / 3.00 / 90.3
\\

Grok Voice
& 100.0 / 2.37 / 96.7
& 67.8 / 49.4
& 0.0 / n/a / n/a
& 80.5 / 3.13 / 84.0
\\

Qwen3.5-Omni-Flash-Realtime
& 100.0 / 2.41 / 98.3
& 72.5 / 49.6
& 2.2 / $-4.94$ / 66.7
& 91.3 / 2.68 / 84.9
\\

\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table*}

==> Draft-components/history/related_work.tex <==
\begin{table*}[t]
\centering
\caption{
Comparison of existing benchmarks.
Action coverage: $\checkmark$ explicitly covered;
$\circ$ related coverage via conditions, design, or evaluation\td{partial coverage?};
$\times$ no coverage.
Scenarios: C = casual conversation, S = customer service,
I = interview, M = meeting; -- = unclassified.
$^{*}$Multi-turn conversations.\td{would the middle part be data, and then divided into real percentage and scenarios?}
}
\label{tab:benchmark_comparison}

\begingroup
\scriptsize
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.0}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\textbf{Benchmark}
& \multicolumn{2}{c}{\textbf{Eval.}}
& \textbf{Real / Total}
& \textbf{Scenario}
& \multicolumn{8}{c}{\textbf{Action Coverage}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){6-13}
& \textbf{Immediate}
& \textbf{Subsequent}
& &
& \textbf{Wait}
& \textbf{Ignore}
& \textbf{Take Turn}
& \textbf{Backch.}
& \textbf{Stop}
& \textbf{Hold Floor}
& \textbf{Recover}
& \textbf{Interrupt} \\
\midrule

FDB-v1
& $\checkmark$ & $\times$ & 54\% / 727 & C
& $\circ$ & $\times$ & $\checkmark$ & $\checkmark$
& $\circ$ & $\times$ & $\circ$ & $\times$ \\

FDB-v1.5
& $\checkmark$ & $\times$ & 0\% / 499 & C
& $\times$ & $\times$ & $\times$ & $\times$
& $\circ$ & $\circ$ & $\circ$ & $\times$ \\

FDB-v2.0
& $\checkmark$ & $\times$ & 0\% / 200$^{*}$ & --
& $\times$ & $\times$ & $\circ$ & $\circ$
& $\circ$ & $\circ$ & $\circ$ & $\times$ \\

FDB-v3.0
& $\checkmark$ & $\times$ & 0\% / 100$^{*}$ & S
& $\times$ & $\times$ & $\circ$ & $\times$
& $\times$ & $\times$ & $\times$ & $\circ$ \\

HumDial-FDBench
& $\checkmark$ & $\times$ & 0\% / 5,000 & --
& $\circ$ & $\circ$ & $\times$ & $\times$
& $\circ$ & $\circ$ & $\circ$ & $\times$ \\

$\tau$-Voice
& $\checkmark$ & $\times$ & 0\% / 278 & S
& $\times$ & $\times$ & $\circ$ & $\times$
& $\circ$ & $\circ$ & $\circ$ & $\circ$ \\

FLEXI
& $\checkmark$ & $\times$ & 0\% / 1,200 & --
& $\circ$ & $\times$ & $\checkmark$ & $\checkmark$
& $\checkmark$ & $\circ$ & $\circ$ & $\checkmark$ \\

FD-Bench
& $\checkmark$ & $\times$ & 0\% / 293$^{*}$ & C
& $\times$ & $\times$ & $\circ$ & $\times$
& $\circ$ & $\circ$ & $\circ$ & $\circ$ \\

MTR-DuplexBench
& $\checkmark$ & $\times$ & 33\% / 600$^{*}$ & C
& $\circ$ & $\times$ & $\checkmark$ & $\checkmark$
& $\circ$ & $\times$ & $\circ$ & $\times$ \\

\midrule
\textbf{\sysname{}}
& $\checkmark$ & $\checkmark$
& \textbf{54\% / 4,691} & \textbf{C,S,I,M}
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\endgroup
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

